Null-stream-based Bayesian Unmodeled Framework to Probe Generic Gravitational-wave Polarizations

We present a null-stream-based Bayesian unmodeled framework to probe generic gravitational-wave polarizations. Generic metric theories allow six gravitational-wave polarization states, but general relativity only permits the existence of two of them namely the tensorial polarizations. The strain signal measured by an interferometer is a linear combination of the polarization modes and such a linear combination depends on the geometry of the detector and the source location. The detector network of Advanced LIGO and Advanced Virgo allows us to measure different linear combinations of the polarization modes and therefore we can constrain the polarization content by analyzing how the polarization modes are linearly combined. We propose the basis formulation to construct a null stream along the polarization basis modes without requiring modeling the basis explicitly. We conduct a mock data study and we show that the framework is capable of probing pure and mixed polarizations in the Advanced LIGO-Advanced Virgo 3-detector network without knowing the sky location of the source from electromagnetic counterparts. We also discuss the effect of the presence of the uncaptured orthogonal polarization component in the framework, and we propose using the plug-in method to test the existence of the orthogonal polarizations.

==> sections/experiment.tex <==
\section{experiment}


==> sections/projection_based_inference.tex <==
\section{Projection-based Inference}
\label{sec:proj_based_inference}
The property of polarization type dependent but waveform independent construction of $\boldsymbol{P}$ hints the possibility to infer the polarization content of the observed signal without assuming the waveform model. The inference which based on projection is distinct from the typical Bayesian model selection problems in GW data analysis which compare evidences of different assumed waveform models. Usually, we assume the detector noise follows a stationary Gaussian distribution \cite{Abbott_2020_guide}, and therefore in the Fourier domain we have the Whittle likelihood (cite something) which takes the form
\begin{equation}
	\label{eq:usual_likelihood}
	p(\tilde{\boldsymbol{d}}|\boldsymbol{\theta};\mathcal{H}) \propto \exp\left(-\frac{1}{2}(\tilde{\boldsymbol{d}}-\tilde{\boldsymbol{h}}(\boldsymbol{\theta})|\tilde{\boldsymbol{d}}-\tilde{\boldsymbol{h}}(\boldsymbol{\theta}))\right)
\end{equation}
where $\tilde{\boldsymbol{d}}$ is the observed data, $\tilde{\boldsymbol{h}}(\boldsymbol{\theta})$ is the waveform with parameters $\boldsymbol{\theta}$, and $(\cdot|\cdot)$ denotes the noise-weighed inner product \cite{Abbott_2020_guide}. The model evidence $Z$ is then computed by marginalizing the joint distribution $p(\tilde{\boldsymbol{d}},\boldsymbol{\theta};\mathcal{H})=p(\tilde{\boldsymbol{d}}|\boldsymbol{\theta};\mathcal{H})p(\boldsymbol{\theta};\mathcal{H})$ over all model parameters
\begin{equation}
	Z = \int p(\tilde{\boldsymbol{d}}|\boldsymbol{\theta};\mathcal{H})p(\boldsymbol{\theta};\mathcal{H})d\boldsymbol{\theta}\,.
\end{equation}
The likelihood in Eq.~(\ref{eq:usual_likelihood}) describes the consistency of the residual $\tilde{\boldsymbol{d}}-\tilde{\boldsymbol{h}}(\boldsymbol{\theta})$ with noise. However, the null projection does not only remove the signal content but also the entire subspace spanned by $\boldsymbol{f}_{m}$, and therefore we would be comparing the consistency of the residual with the noise in the lower dimensional space. The reduced dimensionality of null stream demonstrated in Fig.~\ref{fig:null_stream_demo} could be readily seen by performing a rotation to orient the residual $\tilde{\boldsymbol{z}}$ along the principal axes of $\boldsymbol{I}-\boldsymbol{F}_{w}(\boldsymbol{F}_{w}^{\dagger}\boldsymbol{F}_{w})^{-1}\boldsymbol{F}_{w}^{\dagger}$. Since when the null operator is constructed with the correct parameters, the residual is
\begin{equation}
	\tilde{\boldsymbol{z}}=(\boldsymbol{I}-\boldsymbol{F}_{w}(\boldsymbol{F}_{w}^{\dagger}\boldsymbol{F}_{w})^{-1}\boldsymbol{F}_{w}^{\dagger})\boldsymbol{\mathcal{T}}\left(\tilde{\boldsymbol{n}}_{w};\Delta\boldsymbol{t}\right)
\end{equation}
, and then we perform the singular value deomposition on each frequency bin of $\boldsymbol{I}-\boldsymbol{F}_{w}(\boldsymbol{F}_{w}^{\dagger}\boldsymbol{F}_{w})^{-1}\boldsymbol{F}_{w}^{\dagger}$
\begin{equation}
	(\boldsymbol{I}-\boldsymbol{F}_{w}(\boldsymbol{F}_{w}^{\dagger}\boldsymbol{F}_{w})^{-1}\boldsymbol{F}_{w}^{\dagger})[k] = \boldsymbol{U}_{k}\boldsymbol{\Sigma}_{k}\boldsymbol{V}^{\dagger}_{k}
\end{equation}
where $\boldsymbol{U}_{k}\in\mathbb{C}^{D\times D}$ is a unitary matrix, $\boldsymbol{\Sigma}_{k}\in\mathbb{R}^{D\times D}$ is a diagonal matrix with the singular values as the diagonal entries, $\boldsymbol{V}_{k}\in\mathbb{C}^{D\times D}$ is a unitary matrix, and the subscript $k$ denotes the decomposition of the $k^{\text{th}}$ frequency component of the projector $\boldsymbol{I}-\boldsymbol{F}_{w}(\boldsymbol{F}_{w}^{\dagger}\boldsymbol{F}_{w})^{-1}\boldsymbol{F}_{w}^{\dagger}$. The residual along the principal axes could be obtained by
\begin{equation}
	\tilde{\boldsymbol{z}}_{\text{rotated}}[k] = \boldsymbol{U}_{k}^{\dagger}\tilde{\boldsymbol{z}}[k]\,.
\end{equation}
Fig.~\ref{fig:null_stream_demo} demonstrates an example of null projection. For the sake of a more intuitive demonstration, the data are displayed in the time domain. The figures in the left panel show the observed strain outputs with a pure tensorial GW buried in noise. The figures in the middle panel show the residuals after applying the null operator constructed with $\boldsymbol{F}=\begin{bmatrix}\boldsymbol{f}_{+}& \boldsymbol{f}_{\times}\end{bmatrix}$. One should notice that the signal content is removed and the amplitude of the residual is reduced compared to the strain outputs. This is due to the reduced dimensionality after applying the null operator. The reduced dimensionality could be observed more readily by orienting the residuals along the principal axes. As expected, since the null operator projects the data from $\mathbb{C}^{D\times K}$ to $\mathbb{C}^{(D-2)\times K}$ ($M=2$ since we have two column vectors in $\boldsymbol{F}$), only the first principal axis contains non-zero entries.

The reduced dimensionality $\mathbb{C}^{(D-M)\times K}$ is determined by the number of column vectors in $\boldsymbol{F}$. Due to the difference in the dimensionality of the residuals, we could not simply perform the usual Bayesian model selection by replacing different constituent $\boldsymbol{f}_{m}$ in $\boldsymbol{F}$ if the residuals are of different dimensionalities. In the following section, we discuss the method we developed to circumvent this difficulty.
